Graph Learning-based Fleet Scheduling for Urban Air Mobility under Operational Constraints, Varying Demand & Uncertainties

This paper develops a graph reinforcement learning approach to online planning of the schedule and destinations of electric aircraft that comprise an urban air mobility (UAM) fleet operating across multiple vertiports. This fleet scheduling problem is formulated to consider time-varying demand, constraints related to vertiport capacity, aircraft capacity and airspace safety guidelines, uncertainties related to take-off delay, weather-induced route closures, and unanticipated aircraft downtime. Collectively, such a formulation presents greater complexity, and potentially increased realism, than in existing UAM fleet planning implementations. To address these complexities, a new policy architecture is constructed, primary components of which include: graph capsule conv-nets for encoding vertiport and aircraft-fleet states both abstracted as graphs; transformer layers encoding time series information on demand and passenger fare; and a Multi-head Attention-based decoder that uses the encoded information to compute the probability of selecting each available destination for an aircraft. Trained with Proximal Policy Optimization, this policy architecture shows significantly better performance in terms of daily averaged profits on unseen test scenarios involving 8 vertiports and 40 aircraft, when compared to a random baseline and genetic algorithm-derived optimal solutions, while being nearly 1000 times faster in execution than the latter.

==> backup/body_backup.tex <==
\section{Introduction}\label{sec:Introduction}
The concept of Urban Air Mobility (UAM) utilizes electric vertical take-off and landing (eVTOL) aircraft \cite{FAA_CON_OPS} to offer automated air transportation for passengers, cargo, and critical (e.g., air-ambulance) services, with a projected global market size of \$1.5 trillion by 2040 \cite{iii, jonas_jonas}. The economic viability of this new mode of transportation depends on the ability to operate a sufficiently large number of increasingly autonomous eVTOLs in any given market (high penetration), which in turn demands safe airspace management and robust fleet planning solutions among others. 
More specifically, deploying a regional UAM network comprising scores of eVTOL aircraft requires an effective scheduling framework that can adapt to the unique demand patterns (different from general aviation) and aircraft and airspace constraints (distinct from other modes of regional/metropolitan transportation), while maximizing profitability and mitigating energy footprint \cite{Hwang2001}. These scheduling problems usually take the form of complex nonlinear Combinatorial Optimization (CO) problems, which can be addressed through classical optimization, heuristic search, and learning-based approaches. Approaches that provide local optimal solutions for small UAM fleet scheduling problems \cite{8569225, Shihab2020OptimalEF, 8901431} often present computational complexity that makes them impractical for online decision-making. By taking a multi-agent task planning perspective of the online fleet scheduling problem, in this paper, we propose a new reinforcement learning (RL) based solution that also accounts for important problem complexities and constraints (often overlooked by existing methods), such as those related to airspace corridors, aircraft charging, vertiport capacity, weather-induced uncertainties, and time-varying demand \cite{FAA_CON_OPS}.

The deployment of a successful UAM network requires a fleet scheduling framework that can address several challenges. These challenges include: 

\textbf{Dynamic environment:} The scheduling framework needs to consider real-time factors such as airspace congestion, weather conditions, ground traffic, infrastructure availability, and demand uncertainty. Thus, adaptive (shorter time-scale and robust) planning is favored over fixed, deterministic, and/or day-ahead planning. It is also computationally challenging to resolve uncertainties in online optimizations.

\textbf{Conflict resolution:} 
The framework should facilitate sharing eVTOLs' state information and allow for trajectory and speed adjustments to ensure safe and optimal sharing of the airspace, which introduces additional constraints on decision-to-fly actions (between any two vertiports).

\textbf{Optimization \& Resource Allocation:} 
Optimizing (scarce) resource allocation, such as vertiport parking slots, charging stations, and air corridor capacity, is essential to prevent unnecessary delays in charging, takeoff, and other operations, which in turn add more constraints on scheduling actions.

\textbf{Learning \& adaptation:} Capability of learning from past experiences, interactions, and feedback to adapt their decision-making strategies is needed. Learning algorithms facilitate agent adaptation to changing conditions, leading to improved efficiency and enhanced system performance by shifting the computational expense of training offline. Similar challenging characteristics can be found in other fleet planning and multi-robot transport or fulfillment planning problems.

To address the stated problem complexities and provide efficient online-executable policies for fleet scheduling, we explore the use of specialized Graph Neural Networks (GNNs) \cite{capam_mrta, paul2022scalable}. Our approach builds upon existing work in multi-robot task allocation and demonstrates superior performance compared to standard RL-based and heuristic optimization-based solutions, as well as a feasible-random baseline, through numerical experiments.

\textbf{Related Work:}\label{sec:Related_works}
There is a small but fast-growing body of work in UAM fleet planning, which has provided impetus for transitioning optimization and learning formalism to advance this emerging concept. However, the majority of the existing work overlooks some of the important guidelines proposed by the FAA \cite{FAA_CON_OPS} w.r.t. UAM airspace integration. Some of these works lack considerations for air corridors, range/battery capacity constraints, and unforeseen events such as route closures (attributed to bad weather or off-nominal events) or dysfunctional eVTOLs \cite{9482700, fernando2023graph, paulaviation2022, 8901431}. Traditional methods such as Integer Linear Programming (ILP) and metaheuristics are not suitable for solving related NP-hard fleet scheduling problems in a time-efficient manner \cite{peng2021graph, miller1960integer, kamra2015mixed, Rizzoli2007, 7462285, zhang1999team, gen-2}. For perspective, here we consider hour-ahead planning, in order to enable enough capacity to adapt to varying demand and state of routes affected by weather and unanticipated aircraft downtime. Learning-based methods have in recent years shown promise for generating policies for CO problems with relatable characteristics \cite{Kool2019, barrett2019exploratory, khalil2017learning, Kaempfer2018LearningTM, 9750805, li2018combinatorial, nowak2017note, Tolstaya2020MultiRobotCA, Sykora2020, Dai2017, capam_mrta}. In their current form, however, they consider fewer complexities or tackle simpler problem scenarios. %Multi-agent Reinforcement Learning (MARL) approaches are another potential solution approach in this context, but are observed to have limited scalability and are affected by non-stationarity issues, making them less suitable for scheduling applications \cite{fernando2023graph, noureddine2017multi}. Moreover, for UAM fleet planning, a centralized decision-making is deemed more practical and (safety-wise) risk averse (as impact of imperfect communication are minimal at hour-ahead fleet planning scale), further limiting the potential suitability of decentralized MARL type approaches \cite{FAA_CON_OPS}.

We propose a centralized learning-based approach to tackle the complexities and safety guidelines in UAM fleet scheduling. Our approach involves creating a simulation environment that incorporates these complexities, and thereof support the training of a policy network for generating (hour-ahead) sequential actions for eVTOLs over a generic (12-hr) day of operation. The policy network combines a Graph Capsule Convolutional Neural Network (GCAPCN) \cite{Verma2018} to encode vertiport and eVTOL state information (both abstracted as graphs), a Transformer encoder network to incorporate time-series data on demand and fare (similar to \cite{chuwang2022forecasting}), and a feedforward network to encode passenger transportation cost. Additionally, a Multi-head Attention mechanism is used to fuse the encoded information and problem-specific context, aiding sequential decision-making \cite{Verma2018, VaswaniSPUJGKP17, Kool2019}.

\textbf{The Main Contributions} 
of this paper can be summarized as \textbf{1)} Formulating the UAM fleet scheduling problem as a Markov Decision Process (MDP), and architecting a centralized encoder-decoder policy network, where the state of the UAM network (vertiports and aircrafts) is embedded by a Graph Neural Network (GNN), with the demand, passenger fare, operating cost and air corridor availability information processed by different Context encoders and then concatenated. The scheduling actions are computed using a Multi-head Attention (MHA) based action decoder, that is fed by the GNN and context. \textbf{2)} Integrating the encoder-decoder policy network with a new simulation environment that models the daily operation of 40 eVTOLs across 8 vertiports, associated uncertainties, and airspace/aircraft constraints, and provides data on demand, fare, and operational costs. \textbf{3)} Training the encoder-decoder network via policy gradient techniques and demonstrating its ability to generalize across unseen scenarios and uncertainties without retraining. \textit{We expect that the new policy architecture presented here can generalize (with minor changes to the Context) to a wider range of multi-agent/vehicle/robot scheduling problems with similar complex characteristics, namely graph-abstractable task/resource space, time-varying and uncertain environment properties, and the need for sequential actions that satisfy a large set of physical and operational constraints.}  %\textbf{4)} Developing a framework with a simulated environment for UAM fleet scheduling operations, incorporating time-varying demand, passenger cost, uncertainties, and constraints guided by FAA guidelines \cite{FAA_CON_OPS, Vertiport_design_FAA}.

\textbf{Paper Outline:} The next section describes the UAM fleet scheduling problem and its MDP formulation. Section \ref{sec:Proposed_solution} explains the proposed solution, including the state encoding and action decoding. Section \ref{sec:experimental_evaluation} covers training and experimental evaluations, and Section \ref{sec:conclusion} presents concluding remarks.

 \begin{figure}[!ht]
    \centering
    \includegraphics[width=.5\textwidth]{Figures/Decision_making.pdf}
    \caption{The trained policy implemented on the UAM network: The two images show two consecutive decision-making instances. For clarity of illustration, only 4 eVTOls are shown.}
    \label{fig:decision-making} 
\end{figure}


\section{Problem Description and Formulation}\label{sec:Problem_description_formulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{itemize}
%     \item X hour ahead scheduling (this will be from learned model)
%     \item After a cancellation of flight, reschedulling is required - this should be mentioned in the testing
%     \item Mention that the features, complexities, and constraits considered are based on the FAA conops document, and the one from Boeing
% \end{itemize}

% \textcolor{red}{Write about rebalancing (space-driven or demand-driven)}

A UAM network includes vertiports and eVTOLs for passenger transportation, with vertiports serving as charging spots, parking areas, and terminals for passenger boarding and departing. 
We consider a concept of operations (ConOps), where every vertiport is connected to each other (i.e., a \textit{fully} connected vertiport network \cite{9925782}) by a route that comprises air corridors (as shown in Fig. \ref{fig:decision-making}); for safe operation, eVTOLS can only use these air corridors for flight. Since a real-world functioning UAM network is not yet functional, the vertiport connection could be fully connected or just connected (or partial) vertiports, and the proposed approach can also be extended for connected (or partially connected) vertiports. A fully connected network is where all the nodes are connected to each other, while in a connected network, there exists a direct or indirect (multi-hop) connection between two nodes. The corridors have regulations regarding the required distance gap for safe navigation. Here, we consider the corridors to be straight tube-shaped air columns. We consider there to be 4 air corridors between two vertiports with two corridors for each direction. The UAM network is defined as involving $N$ vertiports, and $N_{K}$ number of eVTOLs, with each eVTOL having a maximum passenger seating capacity of $C$ (=4) and maximum battery capacity of $B_{\text{max}}$ (=110kWh). Let $V$ and $K$ be the set of all vertiports and eVTOLs, respectively. Each vertiport $i \in V$ has a maximum number ($C^{\text{park}}_{\text{max}}$=10) of eVTOLs it can accommodate/park at a time and a maximum number of charging stations ($C^{\text{charge}}_{\text{max}}$=6) it contains. Some of the vertiports that do not have a charging facility called vertistops ($V_{s} \subset V$) are only used for landing/take-off, and passenger boarding and have parking spaces. For computing the cost of transportation, we define $R_{i,j}$ to be the cost of transporting a passenger from vertiport $i$ to $j$. The travel demand between vertiports is modeled based on real data as explained in Section \ref{subsec:Demand_model}. Each vertiport $i \in V$, has an expected take-off delay $T^{\text{TOD}}_{i}$ which will affect every take-off from the vertiport during an episode. Here, an episode refers to the UAM operation for a specific time period.

We make the following assumptions for setting up this problem:
    \textbf{1)} A single service provider runs the entire UAM network, and full observation of the states of aircraft and vertiports in the network is available to the central agent making the scheduling decisions (reasonable under current communication capabilities, given planning occurs here at 15-60 min time scales). 
    \textbf{2)} Every eVTOL can commute between any two vertiports if it has enough battery charge (considering a safety margin) for the commute.
    \textbf{3)} The resistive loss of the batteries is negligible.
    \textbf{4)} The state information of eVTOLs and vertiports is always accessible for decision-making, which is crucial for ensuring passenger safety in aviation applications.
    \textbf{5)} An estimate of the probability of unplanned technical grounding of eVTOLs is available.
    \textbf{6)} While route closure on a given day of operation is not known apriori, an estimate of the probability of route closure (due to factors such as bad weather) is however available.
    \textbf{7)} The expected take-off delay ($T^{\text{TOD}}_{i}, i \in V$) at every vertiport can be estimated and is considered to be less than 6 minutes.
 We consider a probability of route closure between two vertiports $P^{\text{closure}}_{i,j} (\leq 0.05), \forall i, j \in V$. Once the route is closed, there will not be any more commutes between these two vertiports during the rest of the episode. We consider the probability of an eVTOL to become dysfunctional $P_{k}^{\text{fail}} (\leq .005), \forall k \in K$ during an episode. For every episode, we consider an expected take-off delay for all the vertiports, which are assigned randomly (< 30 minutes). During take-off from a vertiport $i \in V$, we consider a random delay following a Gaussian distribution with mean $T^{\text{TOD}}_{i}$ and a standard deviation of 6 minutes. We assume this expected take-off delay to be known prior to the scheduling. While these uncertainties are modeled for realism, and seeded with prescribed values as there is no significant historical data in this regard, these values can be readily tweaked once data (or forecasts) become available. Passenger pricing for a journey is based on operational cost per passenger and the demand for the trip. Upon reaching a vertiport, each eVTOL is fully charged before proceeding to the next destination (excluding vertistops) or being parked in an available spot if it is idle.
 

The planning objective is to maximize daily profit by optimizing the schedule of eVTOL flights between vertiports to meet travel demand. Each decision-making instance involves assigning an eVTOL (currently at a vertiport) to another vertiport to fly to or instructing it to remain idle for another 15 minutes. Factors such as demand, battery charge, and operational costs are taken into account. The current implementation focuses on a 4-hour episode between 6 am and 6 pm without an end-of-episode constraint. Each episode is independent, starting with a random number of fully charged eVTOLs at each vertiport, considering vertiport capacity constraints. The passenger demand model, eVTOL battery model, and optimization formulation of the problem are further discussed. The detailed optimization formulation can be found in Section \ref{subsec:optimization_formulation}.

\subsection{Demand Model}\label{subsec:Demand_model}
 Passenger demand modeling is used to generate stochastic passenger requests between different vertiports. The demand is based on forecasted data from \cite{Administration}, and we assume knowledge of the demand for each hour during daily operating hours. The demand between two vertiports $i$ and $j$ at a time t $Q(i,j,t)$ mimics the demand patterns of a major city's subway system, where certain stations representing offices and workplaces experience higher traffic. In our scenario, a subset of vertiports $V_{B} \subset V$ is designated as high-demand vertiports. The demand between vertiports in $V_{B}$ is higher compared to those in $V - V_{B}$. We consider two peak hours: $8-9am$ ($T^{\text{peak}1}$) and $4- 5pm$ ($T^{\text{peak}2}$). Vertiports in $V_{B}$ experience peak demand during both hours, resembling the morning and evening rush hours for commuting between home and workplace. The journey demands from vertiports in $V - V_{B}$ to those in  $V_{B}$ peak during $T^{\text{peak}1}$, while the opposite is true during $T^{\text{peak}_2}$, reflecting the rush hour commute from workplace to home.  
 % \begin{equation}
 %     Q(i,j,t) = 
 %     \begin{cases}
 %    \mathcal{N}(100, 10) \ i \in V_B, j \in V_B i\neq j, \ t =T^{\text{peak}_1} \ \\ or \ t=T^{\text{peak}_2} \\
 %    \mathcal{N}(100, 10) \ i \in V-V_B, j \in V_B, i\neq j, \ \\ t =T^{\text{peak}_1} \ \\
 %    \mathcal{N}(100, 10) \ i \in V_B, j \in V-V_B, i\neq j,  \ \\ t=T^{\text{peak}_2} \\
 %    \mathcal{N}(50, 10) \ i \in V_B, j \in V_B, i\neq j, \ t \neq T^{\text{peak}_1} \ \\ and \ t \neq T^{\text{peak}_2} \\
 %    \mathcal{N}(30, 5) \ \text{otherwise}
 %     \end{cases}
 % \end{equation}
 % where $\mathcal{N}(\mu, \sigma)$, represents a normal distribution with mean $\mu$ and standard deviation $\sigma$.
\subsection{eVTOL model}\label{subsec:eVTOL_model}
The eVTOL vehicle model considered here is the same as in \cite{paulaviation2022} (City Airbus eVTOL aircraft), having a maximum cruise speed of $74.5 \ \text{mph}$, maximum passenger capacity of $4$, and with a maximum range of $50$ miles The operating cost of the vehicle is about $\$0.64$ per mile \cite{Shihab2020OptimalEF}. We also assume that for every eVTOL $k$ a (downtime) probability of being dysfunctional given by $P_{k}^{\text{fail}}$, based on work on aircraft predictive maintenance \cite{schoppmann2022operation}. Once an eVTOL become dysfunctional, it can no longer be in service for the remainder of the episode. The battery model is considered to be the same as that in \cite{paulaviation2022}, which consists of a maximum capacity $B_{\text{max}}$= 110 kWh. If $B^{k}_{t}$ is the battery charge of eVTOL $k$ at time $t$, and assuming the eVTOL travels from vertiport $i$ to $j$, the charge for the next time step $B^{k}_{t+1}$ can be computed as $B^{k}_{t+1} = B^{k}_{t} - B^{\text{charge}}_{i,j}$, where $B^{\text{charge}}_{i,j}$ is the charge required to traverse between vertiports $i$ and $j$. The batteries are charged at the vertiports with a charging rate of 150 kW.

\subsection{Passenger Fare Pricing Model 
 \& Electricity pricing}
The passenger price consists of a fixed base fare $F^{\text{base}}$ of $\$5$ and a variable fare $F^{\text{passenger}}$. The variable fare between two vertiports for a passenger at a time $t$ $F^{\text{passenger}}_{i,j,t}$ is computed as a function of the demand profile $Q(i,j,t)$ and the operational cost $R_{i,j}$ (between i and j) as $F^{\text{passenger}}_{i,j,t} = R_{i,j} \times Q_{\text{factor}}(i,j,t)$, where $Q_{\text{factor}}(i,j,t) = \text{max}(\text{log}(Q(i,j,t)/10), 1)$.
This is a hand-made function to account for demand in passenger pricing.
The electricity pricing, $\text{Price}^{\text{elec}}$ is a constant price of $20$ cents per kilowatt-hour \cite{electric_price}.

\subsection{Optimization Formulation}\label{subsec:optimization_formulation}

The fleet scheduling problem becomes a stochastic INLP due to uncertainties such as route closures, eVTOL malfunctions, and expected delays. Consider a time period $T$ (with $|T|$ hours), with a start time of $T^{\text{start}}$ and end time of $T^{\text{end}}$. We consider cases where $T^{\text{end}}$ $<$ $6pm$, and $T^{\text{start}}$ = $T^{\text{end}} - |T|$, and $T^{\text{start}}$ $\geq$ $6am$. For every eVTOL $k \in V_{e}$, let $S^{\text{jour}}_{k}$ be the set of journeys taken during the time period of $T$ (this could be of different length for different eVTOLs). Let $N_{i,l}^{\text{passengers}}$ be the number of passengers transported during the trip $l \in S^{\text{jour}}_{k}$ by eVTOL $k$. Let $B^{k}_{l}$ be the battery charge of eVTOL $k$ just before its $l$'th journey, $V^{\text{start}}_{k,l}$ and $V^{\text{end}}_{k,l}$ be the start and end vertiports of eVTOL $k$ during its $l$'th journey, $T^{\text{takeoff}}_{k,l}$ and $T^{\text{landing}}_{k,l}$ be the takeoff time and landing time of eVTOL $k$ during its $l$'th journey.

Therefore, the total cost of transportation ($\text{Cost}^{\text{Oper}}$) and charging ($\text{Cost}^{\text{Elec}}$) and the revenue during $T$,is given by:
\begin{equation}\label{eq:cost_oper}
% \footnotesize
    \text{Cost}^{\text{Oper}} =  \sum_{k \in K} \sum_{l \in S^{\text{jour}}_{k}} N_{i,l}^{\text{passengers}} \times R_{i,j} , \ i = V^{\text{start}}_{k,l}, \ j = V^{\text{end}}_{k,l}
\end{equation}

\begin{equation}\label{eq:cost_elec}
% \footnotesize
\text{Cost}^{\text{Elec}} = \sum_{k \in K} \sum_{l \in S^{\text{jour}}_{k}} \text{Price}^{\text{elec}} \times B^{\text{charge}}_{i,j}, \ i = V^{\text{start}}_{k,l}, \ j = V^{\text{end}}_{k,l} 
    % C^{C} = \sum_{jk \in J_{k}}  \sum_{k \in K}  \text{Price}^{elec}}_{t} g_{i,j,k}, \ i = Loc^{k}_{\text{start}}(jk), \ j = Loc^{k}_{\text{end}}(jk)
\end{equation}
%
%
\begin{align}\label{eq:revenue}
% \footnotesize
\text{Revenue} = \sum_{k \in K} \sum_{l \in S^{\text{jour}}_{k}} N^{\text{passengers}}_{i,l} \times F^{\text{passenger}}_{i,j,t}, \\ \nonumber \ i = V^{\text{start}}_{k,l}, \ j = V^{\text{end}}_{k,l}, \ t =T^{\text{takeoff}}_{k,l} 
    % R^{T} = \sum_{jk \in J_{k}} \sum_{k \in K} N^{P}_{k}(jk) P_{ijt}, \ i = Loc^{k}_{\text{start}}(jk), \ j = Loc^{k}_{\text{end}}(jk)
\end{align}

Therefore, the objective function can be formulated as:
\begin{equation} \label{eq:objective_function}
% \footnotesize
    \max z = \text{Revenue} - \text{Cost}^{\text{Oper}} - \text{Cost}^{\text{Elec}} 
\end{equation}
Subjected to the following operational constraints:
\begin{gather}
% \scriptsize
    N_{i,l}^{\text{passengers}} = \min(C, Q_{act}(i,j,t)), \\ \nonumber
    i = V^{\text{start}}_{k,l}, \ j = V^{\text{end}}_{k,l}, \ t =T^{\text{takeoff}}_{k,l} \ \forall l \in S^{\text{jour}}_{k} \label{c1} \\
    B^{k}_{T^{\text{takeoff}}_{k,l}} > B^{\text{charge}}_{i,j},\ i = V^{\text{start}}_{k,l}, \ \\ \nonumber j = V^{\text{end}}_{k,l}, \ \forall k \in K, \ \forall l \in S^{\text{jour}}_{k} \label{c2} \\
    C^{\text{park}}_{i,t} <= C^{\text{park}}_{\text{max}}, \ \forall i \in V_{v} \ \forall t \in [T^{\text{start}}, T^{\text{end}}]  \label{c3} \\
    V^{\text{end}}_{l,k} \neq i, \ {\text{if}} \ A^{i, V^{\text{end}}_{l,k}} =0 \ \forall i \in V_{v}, \ \forall k \in K, \ \forall l \in S^{\text{jour}}_{k}\label{c4}
\end{gather}
%
Here $B^{\text{charge}}_{i,j}$ is the amount of charge required for an eVTOL to fly from vertiport $i$ to $j$, $Q_{act}(i,j,t)$ is actual demand (sampled from $Q$), $P^{\text{closure}}$ represents the probability matrix for route closure, and $A$ is a binary matrix such that $A_{i,j} = A_{j,i}=0$ if the route between vertiports $i$ and $j$ is closed. Equations \ref{eq:cost_oper}, \ref{eq:cost_elec}, and \ref{eq:revenue} are used to compute the objective function (Eq. \ref{eq:objective_function}). Equation \ref{c1} is used to compute the number of passengers transported by eVTOL $k$ on its $l$th journey. Constraint \ref{c2} ensures that eVTOL $k$ has enough charge before taking off for its $l$th journey. Constraint \ref{c3} ensures that the number of eVTOLs parked in every vertiport does not exceed its maximum capacity. Constraint \ref{c4} ensures that infeasible vertiports are not chosen during a decision-making instance. This optimization formulation is being used in one of the comparison methods (Genetic Algorithm).
\subsection{MDP Formulation}\label{subsec:MDP+formulation}
% \begin{itemize}
%     \item Why model as MDP and not Markov games?
%     \item Why centralized decision-making?
% \end{itemize}


In this work, we formulate fleet scheduling as an MDP, where actions are computed sequentially for each eVTOL during its decision-making instance ($t \in [T^{\text{start}}, T^{\text{end}}]$). At each time step, an action is assigned to each eVTOL based on the current network state, which contains all necessary information for decision-making. Unlike other multi-agent approaches in smaller UAM settings, where safety is less critical, UAM requires high safety standards \cite{FAA_CON_OPS}. Therefore, full state information is essential for decision-making, leading us to adopt a centralized decision-making scheme.

\textbf{Graph Formulation for UAM vertiport Network:}
The UAM vertiport network is expressed as a graph $G_{v} = (V_{v},E_{v},A_{v})$, where $V_{v}$ (=$V$) represents the set of nodes or vertiports; in this case, $E_{v}$ represents the set of edges between the nodes, $A_{v}$ represents the adjacency matrix of the nodes. Since we consider a route closure probability $P^{\text{closure}}$, we compute the weighted adjacency matrix as $A_{v} = (\mathbf{1}_{N \times N} - P^{\text{closure}}) \times A$, where $A$ is a matrix representing the route closure such that if $A_{i,j}$ represents the route between nodes $i$ and $j$ ($i,j \in V_{v}$), then $A_{i,j}$ = $A^{j,i}$ = 0 if the route is closed, else it is 1. Here, the properties $\delta^{t}_{i}$ of each node $i \in V_{v}$ at time step $t$ are: \textbf{1)} x-y coordinates of the node/vertiport ($x_{i}, y_{i}$)   \textbf{2)} Number of eVTOLs that are parked at vertiport $i$ at time $t$, $C^{\text{park}}_{i,t}$ \textbf{3)} The earliest time at which a charging station is available $T^{\text{charge}}_{i}$, \textbf{4)} The expected take-off delay $T^{\text{TOD}}_{i}$, \textbf{5)} A binary number $I^{\text{vstop}}_{i}$ which takes a value of 1 if the node is a vertistop. Therefore, $\delta^{t}_{i} = [x_{i}, y_{i}, C^{\text{park}}_{i,t},T^{\text{charge}}_{i}, T^{\text{TOD}}_{i}, I^{\text{vstop}}_{i}]$,  $\delta^{t}_{i}$ $\in$ $\mathbb{R}^{6}$. 

\textbf{Graph Formulation for eVTOLs Network:} The state of eVTOLs can be represented as graph $G_{e} = (V_{e},E_{e},A_{e})$, where $V_{e}$ represents the set of eVTOLs, $E_{e}$ represents the set of edges between the nodes, $A_{e}$ represents the adjacency matrix. We consider $G_{e}$ to be fully connected. Each node $k$ $\in$ $V_{e}$ has its time-varying node properties $\psi^{t}_{k}$. The properties of each eVTOL node are \textbf{1)} The coordinates of the destination vertiport ($x^{d}_{k}, y^{d}_{k}$), \textbf{2)} Current battery level as a fraction $B_{t}^{k}$, \textbf{3)} The next flight time $T^{\text{flight}}_{k}$, \textbf{4)} Next decision-making time $T^{\text{dec}}_{k}$, \textbf{5)} Probability of failure $P_{k}^{\text{fail}}$. Therefore, $\psi^{t}_{k} = [x^{d}_{k}, y^{d}_{k}, B_{t}^{k}, T^{\text{flight}}_{k}, T^{\text{dec}}_{k}, P_{k}^{\text{fail}}]$, ($\psi^{t}_{i}$ $\in$ $\mathbb{R}^{6}$). 


\textbf{State Space:}
The state information which will be used for computing the action at a time step $t$ consists of:
\textbf{1)} Vertiport graph $G_{v}$, \textbf{2)} eVTOLs graph $G_{e}$, \textbf{3)}  Demand profile $Q$, \textbf{4)} Passenger fare $F^{\text{passenger}}$, \textbf{5)} Cost of per passenger transportation $R$, \textbf{6)} Time at which it's safe to launch an eVTOL to the corridors $T^{\text{cor}} \in \mathbb{R}^{N \times N \times 2}$. It should be noted some of the state variable updates such as $T^{\text{flight}}, T^{\text{dec}},T^{\text{charge}}_{i}, T^{\text{TOD}}_{i}$, etc. are not shown in this paper due to space constraints; however, they have been appropriately implemented programmatically in the developed RL environment. To handle the large state space, we use a Graph Neural Network (GNN) to compute a fixed-length feature vector representing the information of vertiports and eVTOLs. The demand profile and passenger fare are modeled as time-series data using a Transformer encoder. The cost of per-passenger transportation is represented by a learned feature vector from a feedforward network. Corridor closure information $T^{\text{corr}}$ is flattened and concatenated with the aforementioned embeddings.

  \textbf{Action Space:}
During each decision-making instance, there will be one eVTOL that will be taking a decision for its next destination and this eVTOL selects an action i.e., where to fly to next, from the action space ($V^{\text{end}}_{k,l}$ $\in$ $V_{v}$), which includes all available vertiports. If an eVTOL chooses the vertiport it is currently located at, it will wait or idle for 15 minutes at the vertiport before taking a new decision.
We also consider a masking mechanism to not select infeasible vertiport journeys. During a decision-making instance for an eVTOL, the vertiports that violate constraints \ref{c1}, \ref{c2}, and \ref{c3} are masked.

  \textbf{Reward:} We consider a delayed reward strategy, where the total reward computed at the end of the episode is the ratio of the profit (Eq. \ref{eq:objective_function}) to the maximum possible episodic profit,
  
  $\sum_{i \in V,j \in V,t \in [T^{\text{start}}, T^{\text{end}}]} (Q(i,j,t) \times F^{\text{passenger}}_{i,j,t})$. 

  \textbf{Transition:} Uncertain route closure and take-off delay, and uncertain variations in demand lead to a stochastic state transition here, which is computed by the simulation. 


\section{Policy Architecture \& Learning Framework}
\label{sec:Proposed_solution}
  % In this work, we develop a learning framework, which will be used to assign actions to the eVTOLs during a decision-making instance. The policy network takes in the state information during each time step and outputs an action for each eVTOL. The policy network consists (shown in figure \ref{fig:policy}) of GNN-based encoders, Transformer network-based encoders, feedforward network, and Multi-head attention (MHA) based decoder. The state information is encoded as learnable fixed-length feature vectors (of length $l_{\text{embed}}$) by the encoder and a context module and will be used by the decoder to compute the action sequentially. Further information regarding the proposed state encoding and action decoding is discussed in the following section.
We develop an RL framework to compute actions for individual eVTOLs during decision-making instances. The policy model is triggered when a fully charged eVTOL is waiting to be assigned a destination. If an eVTOL remains grounded due to route closures, destination crowding, or insufficient battery, the policy model is re-queried after a 15-minute wait. The policy network takes the state as input and outputs the probability of selecting the next destination for the eVTOL. It combines GNN-based and Transformer-based encoders, a feedforward network, and a Multi-head Attention (MHA) based decoder (Fig. \ref{fig:policy}). The state information is encoded as fixed-length ($l_{\text{embed}}$)  feature vectors using encoders and a context module. These vectors are used by the decoder to compute actions sequentially. Each component of the policy model is further explained below.

\subsection{State Encoding}  

  The state information consists of the information of UAM vertiports, eVTOLs, passenger demand, passenger fare, passenger transportation costs, and electricity pricing. This section describes how the state information is encoded.

\subsubsection{Vertiport and eVTOL State Encoding with GNN:} \label{Sec:GCAPCN} We use a GNN to compute feature vectors for the vertiport and eVTOL state information, both of which are abstracted as graphs. Specifically, we employ a Graph Capsule Convolutional Neural Network (GCAPCN) for learning local and global structures with node properties. The node embedding in GCAPCN is permutation invariant, similar to the approach described in \cite{paulaviation2022}. GCAPCN is a GNN introduced in \cite{Verma2018} to address the limitations of Graph Convolutional Neural Networks (GCN), enabling the encoding of global information using capsule networks as presented in \cite{Hinton}. Further description of the GCAPCN architecture can be found in \cite{paulaviation2022}. We use GCAPCN to
compute node embeddings for the vertiport and eVTOL graphs, $F_{e} \in \mathbb{R}^{N_{K} \times l_{\text{embed}}}$ and $F_{v}\in \mathbb{R}^{N \times l_{\text{embed}}}$ respectively, where $l_{\text{embed}}$ is the embedding length. 
\begin{figure}[!t]
    \centering
    \includegraphics[width=.5\textwidth]{Figures/Policy.pdf}
    \caption{
The CapTAIN policy network consists of state encoders and a decoder, with the state input format. Green and blue blocks represent the policy network and the state space, respectively.}
    \label{fig:policy}
\end{figure}
  
\subsubsection{Transformer-based Encoding of Demand \& Passenger Fare: }\label{subsubsec:transformer_timeseries} In this work, we utilize a Transformer Architecture to compute learnable embeddings for entities that can be represented as time-series data, such as demand distribution over time and passenger fare. The Transformer architecture, originally introduced in \cite{Vaswani2017} and widely used in applications such as Natural Language Processing \cite{Vaswani2017} and time series forecasting \cite{zhou2021informer}, follows an encoder-decoder approach based on self-attention. The encoder maps an input sequence to continuous representations, and the decoder generates an output sequence by attending to relevant information. In our work, we utilize the Transformer encoder to compute continuous and learnable feature vectors for time-series data.
%\subsubsection{Demand distribution and passenger fare encoding}\label{sec:demand_encoding}
%
The forecasted demand between vertiports during each hour ($Q$) and the passenger fare ($F^{\text{passenger}}$) are processed by two separate Transformer networks into learned feature vectors, $F_{Q}\in \mathbb{R}^{l_{\text{embed}}}$ and $F_{P}\in \mathbb{R}^{l_{\text{embed}}}$, respectively.

\subsubsection{Passenger transportation cost encoding:} \label{sec:passenger_transportation_cost_encoding}
The passenger transportation information $(R)$ can be considered as a matrix of size $N \times N$. This information can be encoded as a feature vector $F_{R}$ of length $l_{\text{embed}}$ by passing through a feedforward (FF) network.

\subsubsection{Corridor Availability encoding:}\label{subsubsec:corridor_availability}
For every corridor, we keep track of the time at which it is safe for a new eVTOL to enter the corridor subject to minimum separation requirements governed by safety. The corridor availability $T^{\text{cor}}$, a tensor of size $N \times N \times 2$. $T^{\text{cor}}$ is stretched into a 1-D vector $F_{T}$ of length $N \times N \times 2$, as shown in Fig. \ref{fig:policy}.

\subsubsection{Context:} The context vector is computed by taking the linear transformation of a concatenated vector of the mean of the eVTOL node embedding ($F_{e}$) given by the GCAPCN encoder, the embedding of the eVTOL taking decision ($F_{e}^{k}$), demand and passenger fare encoding given by the transformers ($F_{Q}$ and $F_{P}$), the transportation cost encoding ($F_{R}$) given by the FF, and the corridor availability vector ($F_{T}$). 

\subsection{Action Decoding}
We use a Multi-head Attention-based decoder as shown in Fig. \ref{fig:policy}, to compute which vertiport to visit next, given the vertiport node embeddings ($F_{v}$) and the Context vector. 
The attention mechanism computes compatibility scores between the context and the node embeddings, selecting the destination for the eVTOL based on the highest compatibility score. The choice of the current vertiport itself indicates a stay-idle decision. We call the proposed policy network as \textbf{Cap}sule \textbf{T}ransformer \textbf{A}ttention-mechanism \textbf{I}ntegrated \textbf{N}etwork (\textbf{CapTAIN}).
% \subsection{Training Algorithm} \label{subsec:Training_Algorithm}\vspace{-.2cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Simulation Environment \& Training Algorithm} \label{sec:sim}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We considered a hypothetical area of 50 x 50 sq miles with 8 vertiport locations (Fig. \ref{fig:decision-making}), including 2 vertistops $V_{s}$ (1 and 6). Four vertiports (0,4,6, and 7) were designated as high-traffic ($V_{B}$) due to their increased trip demand. The location of vertiports remained the same for each training scenario, while the hourly demand values changed for each episode. The environment was implemented in Python using the OpenAI Gym interface, making it compatible with RL training algorithms like A2C and PPO through the stable-baselines3 library. To train the policy network, a policy-gradient RL method such as Proximal Policy Optimization (PPO) \cite{schulman2017proximal} or the Actor-Critic method \cite{Konda2003OnActorCriticA} can be used. Here, we use PPO from \textbf{stable-baselines3} \cite{stable-baselines3}. A 2-layer neural network with input and intermediate length $l_{\text{embed}}$ and LeakyReLU activation is used as the value network.
\section{Experimental Evaluation}\label{sec:experimental_evaluation}
% \begin{itemize}
%     \item Training convergence and training time
%     \item Testing for generalizability
%     \item Ablation study
%     \item Analysis of total delay
%     \item if results are close, then do statistical analysis
%     \item Total trips made
%     \item When the probaiblity of route closure is very high. Will the number wait action be more? If yes, it means its a conservative approach.
% \end{itemize}
In order to test the performance of the proposed policy architecture and the impact of the novel encoder choices, we trained 2 other policy networks (on two GPUs (NVIDIA Tesla V100) with 16GB RAM.). The first policy ablates the two GCAPCN encoders by replacing it with a Multi-Layered Perceptron (MLP) and is named the \textbf{Ablation-GCAPCN}, while the second policy ablates the Transformer network by replacing it with an MLP, and is named the \textbf{Ablation-Transformer}. These models are also compared against two other baselines (Section \ref{subsec:generalizability}): 

\textbf{1)} A \textbf{Genetic Algorithm (GA)} with a population size of 30, max iteration of 30, mutation probability of 0.1, elite ratio of 0.1, and crossover probability of 0.5. Here, the GA was implemented in batches of 30 sequential decisions. During each batch, the optimization variables are the 30 decisions where each decision takes an integer value between 1 and N (for each vertiport), and the objective function is computed using Eq. \ref{eq:objective_function} at the end of the 30 decisions. We take the 30 decision variables and run the simulation with these 100 decisions implemented sequentially resulting in an updated environment state. The optimization of the next 30 decisions starts with the current state of the environment. This is continued until the end of an episode.; 

\textbf{2)} A \textbf{Feasibility Preserving Random Walk (Feas-RND)} that selects a feasible vertiport as the next destination during each decision-making instance.

Ablation-GCAPCN, and Ablation-Transformer are considered two learning-based baseline methods, while GA and Feas-RND are two non-learning-based baseline methods.

\subsection{Training \& Convergence}\label{subsec:training_convergence}
\begin{figure}[!t]
    \centering
    \includegraphics[width=.5\textwidth]{Figures/Convergence.pdf}
    \caption{Convergence plot for all the trained models}
    \label{fig:convergence} 
\end{figure}
% \begin{table}[!ht]
\begin{table}[h]
\caption{Training settings}
\label{table:training_algo_info}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lc}
\toprule
 Details &  Values \\ 
\midrule
\textit{Total steps}   & 2e6  \\
\textit{Rollout size}   & 20000   \\
\textit{Optimizer}   & \textit{Adam}  \\
\textit{Learning step} & 1e-7 \\
\textit{Entropy coef} & 0.01  \\
\textit{Value coef} & 0.5  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}
The three policies are trained using PPO for 2 million steps using the parameters in Table \ref{table:training_algo_info}. From the convergence plots in Fig. \ref{fig:convergence}, it can be seen that CapTAIN converges to a higher episodic mean reward compared to the other two policies, while Ablation-Transformer episodic rewards improved until 900K steps, after which the performance started to deteriorate (requires further investigation).
This shows the combination of the two components (GCAPCN and Transformer) has better learning capability. The trained models are tested and the non-learning-based methods (GA and Feas-RND)  are implemented on a 2.6 GHz Intel core i7 MacOS 11.2.3 system.
%


\subsection{Generalizability \& Ablation Study}\label{subsec:generalizability}
The trained RL models and the baselines are tested on 100 unseen episodes. Figure \ref{fig:generalizability} compares the results across all 100 scenarios based on the following metrics: mean episodic reward, episodic profit, \# stay-idle decisions, and \# flight decisions.
\begin{figure}[!t]
    \centering
    \includegraphics[width=.5\textwidth]{Figures/Generalizability.pdf}
    \caption{Comparative analysis of the 5 methods on total episodic reward, total episodic profit, total idle decisions, and total flight decisions.}
    \label{fig:generalizability}
\end{figure}
CapTAIN outperforms GA in terms of the average episodic rewards, achieving a mean reward of .34 (Fig. \ref{fig:generalizability}) compared to GA's mean reward of .29. In order to check if the performance difference between CapTAIN and GA is significant, we performed a statistical T-test (with the null hypothesis being that both the mean is the same), and the $p\text{-value}$ was found to be 6$\times$$10^{-6} (<.05)$, which indicates that there is a significant difference between the performance of CapTAIN and GA. As expected the Feas-RND performed the worst.

The total episodic profit (Fig. \ref{fig:generalizability}) is quite reflective of the episodic reward, and thus the performance ranking of the methods remains the same in terms of profit. Comparing the two ablation networks to CapTAIN (in Fig. \ref{fig:generalizability}), it can be seen that Ablation-Transformer performs poorer compared to Ablation-GCAPCN. This shows that the Transformer encoder contributes more strongly to generalizability compared to GCAPCN, at least under the current problem settings.


\subsubsection{Computation Time analysis}\label{subsubsec:computation_time}
The solution computing time for the GA is determined by adding the total time for which the optimization (in batches) was performed. And similarly for CapTAIN, and the other learning-based methods, the total episodic computing time is the sum of the time for the forward propagation through the policy network throughout an episode. The computing time for all the 100 test scenarios is averaged and compared between all the methods.
 The average episodic computation time required by the GA is about 1,774 seconds, while for CapTAIN, it was only 2.1 seconds.


\subsection{Qualitative analysis of decision-making}\label{subsec:Qualitative analysis}
In order to physically interpret the quality of the decision-making by all the methods, we tracked the total number of idle decisions, the total number of flight decisions, the total episodic flight time, idle time, and delay time for every eVTOL. From Fig. \ref{fig:generalizability}, it can be seen that Feas-RND and GA have comparatively more number of flight decisions and less number of idle decisions, and similarly more episodic flight time per eVTOL and less episodic idle time per eVTOL (Fig. \ref{fig:secondary}), compared to CapTAIN. While further analyses are required, these outcomes might relate to the distribution of flights across peak (high demand/high fare) and off-peak (low demand/low fare) hours, with the CapTAIN network likely learning better tradeoffs to maximize profits. 
Both GA and Feas-RND also have a lower total episodic delay per eVTOL, compared to CapTAIN. This shows that the CapTAIN policy compromises delay with the objective of a higher profit.

\begin{figure}[!t]
    \centering
    \includegraphics[width=.5\textwidth]{Figures/Secondary.pdf}
    \caption{
Comparing the effect of the 5 methods on total idle time, total flight time, and total delay time per eVTOL.}
    \label{fig:secondary}
\end{figure}

\section{CONCLUSIONS} \label{sec:conclusion}

We proposed a graph RL approach using a new encoder-decoder policy architecture to perform UAM fleet scheduling, that uniquely considers uncertainties (in delays, aircraft downtime, and route closures), time-varying demand, vertiport constraints, and airspace constraints. The state of eVTOL aircraft and vertiport occupancy were expressed as graphs, while demand forecast and fares were treated as time-series data. Our novel architecture (CapTAIN) comprises Graph Capsule Convolutional Networks, Transformer encoders, feedforward context layers, and a Multi-head Attention-based decoder to compute sequential actions. Each of these components of CapTAIN is designed to play a specific role that caters to a specific complexity of the fleet scheduling problem, such as scalable embedding of the structural information of the vertiports and eVTOL graphs, and transforming time-series data on demand and passenger fare into context vectors. The policy was trained using PPO and evaluated on 100 unseen scenarios. Compared to non-learning-based methods (GA and Feas-RND), our CapTAIN achieved better performance with up to 3 orders of magnitude faster computation time (than GA). Ablation studies showed that the Transformer encoder had a greater impact on performance than graph neural net encoders. Future directions include extending planning horizons and incorporating end-of-episode constraints to improve the myopic implementation of the policy. Additionally, it explores decentralized policies suitable for scenarios with multiple stakeholders operating vertiports and eVTOL fleets.






% \appendix
% %Appendix A


% \begin{acks}
%   The authors would like to thank Dr. Yuhua Li for providing the
%   matlab code of  the \textit{BEPS} method. 

%   The authors would also like to thank the anonymous referees for
%   their valuable comments and helpful suggestions. The work is
%   supported by the \grantsponsor{GS501100001809}{National Natural
%     Science Foundation of
%     China}{http://dx.doi.org/10.13039/501100001809} under Grant
%   No.:~\grantnum{GS501100001809}{61273304}
%   and~\grantnum[http://www.nnsf.cn/youngscientsts]{GS501100001809}{Young
%     Scientsts' Support Program}.

% \end{acks}

